KHAN: Knowledge-Aware Hierarchical Attention Networks for Accurate Political Stance Prediction

The political stance prediction for news articles has been widely studied to mitigate the echo chamber effect -- people fall into their thoughts and reinforce their pre-existing beliefs. The previous works for the political stance problem focus on (1) identifying political factors that could reflect the political stance of a news article and (2) capturing those factors effectively. Despite their empirical successes, they are not sufficiently justified in terms of how effective their identified factors are in the political stance prediction. Motivated by this, in this work, we conduct a user study to investigate important factors in political stance prediction, and observe that the context and tone of a news article (implicit) and external knowledge for real-world entities appearing in the article (explicit) are important in determining its political stance. Based on this observation, we propose a novel knowledge-aware approach to political stance prediction (KHAN), employing (1) hierarchical attention networks (HAN) to learn the relationships among words and sentences in three different levels and (2) knowledge encoding (KE) to incorporate external knowledge for real-world entities into the process of political stance prediction. Also, to take into account the subtle and important difference between opposite political stances, we build two independent political knowledge graphs (KG) (i.e., KG-lib and KG-con) by ourselves and learn to fuse the different political knowledge. Through extensive evaluations on three real-world datasets, we demonstrate the superiority of DASH in terms of (1) accuracy, (2) efficiency, and (3) effectiveness.

==> Data/fig_eq2.tex <==
\begin{figure}[t]
\begin{tikzpicture}
\centering
\footnotesize
\begin{customlegend}[legend columns=3,legend style={align=center,draw=,column sep=0.5ex}, legend entries={Word2vec, GloVe, ELMo, BERT, RoBERTa, {\m}}]
        \addlegendimage{area legend, red, postaction={pattern=crosshatch dots,pattern color=red}}
        \addlegendimage{area legend, teal, postaction={pattern=north west lines,pattern color=teal}}
        \addlegendimage{area legend, purple, postaction={pattern=grid,pattern color=purple}}
        \addlegendimage{area legend, black, postaction={pattern=vertical lines,pattern color=black}}
        \addlegendimage{area legend, brown, postaction={pattern=horizontal lines,pattern color=brown}}
        \addlegendimage{area legend, blue, postaction={pattern=north east lines,pattern color=blue}}
        \end{customlegend}
\end{tikzpicture}

\begin{subfigure}[b]{0.25\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}, ytick style={draw=none}}
\begin{axis}[
    ybar=3pt,
    bar width=9pt,
    height=3.3cm,
    width=1\linewidth,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    enlarge x limits= 0.6,
    xlabel style={font=\footnotesize},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    % yshift=-5mm,
    ylabel={Train time (sec.)},
    yticklabel style={font=\footnotesize},
    ymin=0, ymax=300,
    yticklabels={0,,100,,200,,300},
    ytick={0,50,100,150,200,250,300},
    xticklabels={},
    xtick=data,
    % symbolic x coords = {SemEval},
    % every node near coord/.append style={rotate=90, anchor=west},
    nodes near coords,
    legend style={
        % nodes={scale=0.5, transform shape},
        % legend image post style={mark=*}
        font=\footnotesize,
        draw=,
        at={(0.415,1.35)},
        anchor=north,
        legend columns=3
        }
    ]
    \addplot+[
        % ybar,
        area legend,
        font=\scriptsize,
        color=red,
    	fill=none, 
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,57)};
    \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=teal,
    	fill=none, 
	    postaction={
            pattern=north west lines, pattern color=teal
        }
    ] coordinates {(0,115)};
    \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=purple,
    	fill=none, 
	    postaction={
            pattern=grid, pattern color=purple
        }
    ] coordinates {(0,193)};
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=black,
    	fill=none, 
	    postaction={
            pattern=vertical lines, pattern color=black
        }
    ] coordinates {(0,244) };
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=brown,
    	fill=none, 
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
    ] coordinates {(0,262) };
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=blue,
    	fill=none, 
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(0,170) };
    % \legend{Word2vec, GloVe, ELMo, BERT, RoBERTa, {\m}}
\end{axis}
\end{tikzpicture}
\vspace{-3mm}
\caption{SemEval}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}, ytick style={draw=none}}
\begin{axis}[
    ybar=3pt,
    bar width=9pt,
    height=3.3cm,
    width=1\linewidth,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    enlarge x limits= 0.6,
    xlabel style={font=\footnotesize},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    yshift=-5mm,
    ylabel={Train time (sec.)},
    yticklabel style={font=\footnotesize},
    ymin=0, ymax=4000,
    yticklabels={0,,1k,,2k,,3k,,4k},
    ytick={0,500,1000,1500,2000,2500,3000,3500,4000},
    xticklabels={,,,},
    xtick=data,
    % symbolic x coords = {AllSides-S},
    % every node near coord/.append style={rotate=90, anchor=west},
    nodes near coords,
    legend style={
        % nodes={scale=0.5, transform shape},
        % legend image post style={mark=*}
        font=\footnotesize,
        draw=,
        at={(0.415,1.35)},
        anchor=north,
        legend columns=3
        }
    ]
    \addplot+[
        % ybar,
        area legend,
        font=\scriptsize,
        color=red,
    	fill=none, 
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,916)};
    \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=teal,
    	fill=none, 
	    postaction={
            pattern=north west lines, pattern color=teal
        }
    ] coordinates {(0,1887)};
    \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=purple,
    	fill=none, 
	    postaction={
            pattern=grid, pattern color=purple
        }
    ] coordinates {(0,2436)};
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=black,
    	fill=none, 
	    postaction={
            pattern=vertical lines, pattern color=black
        }
    ] coordinates {(0,3357)};
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=brown,
    	fill=none, 
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
    ] coordinates {(0,3569)};
        \addplot+[
        % ybar,
        area legend,
    	font=\scriptsize,
        color=blue,
    	fill=none, 
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(0,1795)};
    % \legend{Word2vec, GloVe, ELMo, BERT, RoBERTa, {\m}}
\end{axis}
\end{tikzpicture}
\vspace{-3mm}
\caption{AllSides-S}
\end{subfigure}%
\newline
\begin{subfigure}[b]{0.25\textwidth}
\begin{tikzpicture}[]
\begin{axis}[
    width=1\linewidth,
    height=3.4cm,
    grid=both,
    major grid style={line width=.2pt,draw=gray!50},
    ylabel={Val. Acc.},
    xticklabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize},
    xlabel={\footnotesize Epoch},
    xmin=1, xmax=50,
    ymin=0.5, ymax=1.0,
    xtick={0, 10, 20, 30, 40, 50},
    ytick={0.5,0.6,0.7, 0.8, 0.9, 1.0},
    % yticklabels={0.79, 0.80, 0.81, 0.82},
    % every axis plot/.append style={thick}
    % nodes near coords, 
    % every node near coord/.append style={font=\tiny}
    ]
    \addplot[
        restrict x to domain=0:50,
        each nth point= {1},
        smooth,
        mark=diamond,
        color=red,
        mark size=2pt,
        line width=0.7pt,
        solid,
        ]
    table[x=epoch, y=acc]
    {Data/semeval.txt};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-2mm}
\caption{SemEval}
\end{subfigure}%
\begin{subfigure}[b]{0.25\textwidth}
\begin{tikzpicture}[]
\begin{axis}[
    width=1\linewidth,
    height=3.4cm,
    grid=both,
    major grid style={line width=.2pt,draw=gray!50},
    ylabel={Val. Acc.},
    xticklabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize},
    xlabel={\footnotesize Epoch},
    xmin=1, xmax=50,
    ymin=0.5, ymax=1.0,
    xtick={0, 10, 20, 30, 40, 50},
    ytick={0.5,0.6,0.7, 0.8, 0.9, 1.0},
    every axis plot/.append style={thick}
    % nodes near coords, 
    % every node near coord/.append style={font=\tiny}
    ]
    \addplot[
        restrict x to domain=0:50,
        each nth point= {1},
        smooth,
        mark=triangle,
        mark size=2pt,
        color=blue,
        line width=0.7pt,
        solid
        ]
    table[x=epoch, y=acc]
    {Data/allsides-s.txt};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-2mm}
\caption{AllSides-S}
\end{subfigure}%
\vspace{-3mm}
\caption{The training time and convergence rate with respect to training epochs of {\m} on SemEval and AllSides-S.}\label{fig:eval-performance}
\vspace{-5mm}
\end{figure}



==> Data/fig_eq3.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}
\centering
\small
\begin{customlegend}[legend columns=7,legend style={align=center,draw=,column sep=0.5ex}, legend entries={{\m}-W, {\m}-WS, {\m}-WST, {\m}-All}]
        \addlegendimage{area legend, red, postaction={pattern=crosshatch dots,pattern color=red}}
        \addlegendimage{area legend, teal, postaction={pattern=north west lines,pattern color=teal}}
        \addlegendimage{area legend, brown, postaction={pattern=horizontal lines,pattern color=brown}}
        \addlegendimage{area legend, blue, postaction={pattern=north east lines,pattern color=blue}}
        \end{customlegend}
\end{tikzpicture}
\centering
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
	axis x line*=center,
	axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 100, 200, 300, 400},
    yticklabels={0, 100, 200, 300, 400},
    ymin=0, ymax=400,
    ticklabel style={font=\footnotesize},
    ylabel={Train time (sec.)},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,255.44)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,113.92)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,114.18)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,167.32)};
\end{axis}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
	axis x line=none,
	axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ymin=0.8, ymax=0.96,
    yticklabels={0.80, 0.85 ,0.90, 0.95, 1.00},
    ytick={0.80, 0.85,0.90, 0.95, 1.00},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.8108) (1,0.8278) (2,0.8587) (3,0.9363)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{SemEval ($d=128$)}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 100, 200, 300, 400},
    yticklabels={0, 100, 200, 300, 400},
    ymin=0, ymax=400,
    ticklabel style={font=\footnotesize},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,279)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,137)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,145)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,173)};
\end{axis}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
	axis x line=none,
	axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ymin=0.8, ymax=0.96,
    yticklabels={0.80, 0.85 ,0.90, 0.95, 1.00},
    ytick={0.80, 0.85,0.90, 0.95, 1.00},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.8281) (1,0.8443) (2,0.9180) (3,0.9521)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{SemEval ($d=256$)}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}, ytick style={draw=none}}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 100, 200, 300, 400},
    yticklabels={0, 100, 200, 300, 400},
    ymin=0, ymax=400,
    ticklabel style={font=\footnotesize},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,377)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,246)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,252)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,269)};
\end{axis}
\begin{axis}[
    width=0.96\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
	axis x line=none,
	axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ylabel={Val. Acc.},
    ylabel style={rotate=180},
    ymin=0.8, ymax=0.96,
    yticklabels={0.80, 0.85 ,0.90, 0.95, 1.00},
    ytick={0.80, 0.85,0.90, 0.95, 1.00},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.8196) (1,0.8547) (2,0.9165) (3,0.9427)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{SemEval ($d=512$)}
\end{subfigure}%
\newline    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 1000, 2000, 3000, 4000},
    yticklabels={0, 1k, 2k, 3k, 4k},
    ymin=0, ymax=4000,
    ticklabel style={font=\footnotesize},
    ylabel={Train time (sec.)},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,2313)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,1496)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,1515)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,1770)};
\end{axis}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
	axis x line=none,
	axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ymin=0.7, ymax=0.93,
    yticklabels={0.70, 0.75, 0.80, 0.85, 0.90, 0.95,},
    ytick={0.70, 0.75, 0.80, 0.85, 0.90, 0.95},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.7921) (1,0.8516) (2,0.8742) (3,0.9256)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{AllSides-S ($d=128$)}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\pgfplotsset{xtick style={draw=none}}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 1000, 2000, 3000, 4000},
    yticklabels={0, 1k, 2k, 3k, 4k},
    ymin=0, ymax=4000,
    ticklabel style={font=\footnotesize},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,2701)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,1949)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,2034)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,2237)};
\end{axis}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
	axis x line=none,
	axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ymin=0.7, ymax=0.93,
    yticklabels={0.70, 0.75, 0.80, 0.85, 0.90, 0.95,},
    ytick={0.70, 0.75, 0.80, 0.85, 0.90, 0.95},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.7846) (1,0.8372) (2,0.8594) (3,0.9101)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{AllSides-S ($d=256$)}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
\begin{tikzpicture}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    ybar=0pt,
    enlarge x limits=1.35,
    bar width = 14pt,
    ymajorgrids=true,
    major grid style={line width=.2pt,draw=gray!50},
    xlabel={},
    xlabel style={font=\footnotesize, at={(axis description cs:0.5,0)}},
    xtick align=outside,
    axis x line*=center,
    axis y line*=left,
    xtick pos=left,
    ytick pos=left,
    ytick={0, 1000, 2000, 3000, 4000},
    yticklabels={0, 1k, 2k, 3k, 4k},
    ymin=0, ymax=4000,
    ticklabel style={font=\footnotesize},
    xticklabels={,,,},
    xtick=data,
    nodes near coords,
    ]
    \addplot[
            area legend,
    	font=\scriptsize,
            color=red,
	    postaction={
            pattern=crosshatch dots, pattern color=red
        }
    ] coordinates {(0,3494)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color= teal,  
	    postaction={
            pattern= north west lines, pattern color=teal
        }
    ] coordinates {(1,2769)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=brown,
	    postaction={
            pattern=horizontal lines, pattern color=brown
        }
	] coordinates {(2,3092)};
    \addplot[
    	area legend,
    	font=\scriptsize,
            color=blue,
	    postaction={
            pattern=north east lines, pattern color=blue
        }
    ] coordinates {(3,3383)};
\end{axis}
\begin{axis}[
    width=0.98\linewidth,
    height=3.45cm,
    enlarge x limits= 0.25,
    xtick align=outside,
    axis x line=none,
    axis y line*=right,
    xtick pos=left,
    ytick pos=right,
    ticklabel style={font=\footnotesize},
    ylabel={Val. Acc.},
    ylabel style={rotate=180},
    ymin=0.7, ymax=0.93,
    yticklabels={0.70, 0.75, 0.80, 0.85, 0.90, 0.95,},
    ytick={0.70, 0.75, 0.80, 0.85, 0.90, 0.95},
    xticklabels={,,,},
    xtick=data,
    every axis plot/.append style={thick}
    ]
    \addplot[
        mark=triangle,
        color=black!70,
    ] coordinates {(0,0.7117) (1,0.7412) (2,0.8003) (3,0.9031)};
\end{axis}
\end{tikzpicture}
\centering
\vspace{-3mm}
\caption{AllSides-S ($d=512$)}
\end{subfigure}%
\vspace{-3mm}
\caption{Effectiveness of the main components of {\m} in terms of the training time (bar) and model accuracy (line).}\label{fig:eval-ablation}
\end{figure*}

